Using Synthetic Data for Conversational Response Generation in Low-resource Settings

Response generation is a task in natural language processing (NLP) where a model is trained to respond to human statements. Conversational response generators take this one step further with the ability to respond within the context of previous responses. While there are existing techniques for training such models, they all require an abundance of conversational data which are not always available for low-resource languages. In this research, we make three contributions. First, we released the first Filipino conversational dataset collected from a popular Philippine online forum, which we named the PEx Conversations Dataset. Second, we introduce a data augmentation (DA) methodology for Filipino data by employing a Tagalog RoBERTa model to increase the size of the existing corpora. Lastly, we published the first Filipino conversational response generator capable of generating responses related to the previous 3 responses. With the supplementary synthetic data, we were able to improve the performance of the response generator by up to 12.2% in BERTScore, 10.7% in perplexity, and 11.7% in content word usage as compared to training with zero synthetic data.

==> tables/table5-3.tex <==
\begin{figure*}[!h]
    \centering
    \begin{tabularx}{16cm}{ |p{1.4cm}| X | }
        \hline
        Coverage & Conversation \\
        \hline
       \multirow{4}{\linewidth}{0\%} 
        & \textbf{User:} Kamusta yung weather sa Singapore? Hoping to go there by this year. \\
        & \textbf{DialoGPT:} It's been raining non-stop for the past week and a half. \\
        & \textbf{User:} Ah ganun ba. Hindi na lang ako pupunta if that is the case. \\
        & \textbf{DialoGPT:} I was there last week and i can say that the weather is not that bad. It just rains a lot. \\
        \hline
        \multirow{4}{\linewidth}{10\%}
        & \textbf{User:} Kamusta yung weather sa Singapore? Hoping to go there by this year. \\
        & \textbf{DialoGPT:} Medyo malamig na pero tolerable naman. \\
        & \textbf{User:} Ah ganun ba. Hindi na lang ako pupunta if that is the case. \\
        & \textbf{DialoGPT:} Yup. Malamig talaga. \\ 
        \hline
        \multirow{4}{\linewidth}{15\%} 
        & \textbf{User:} Kamusta yung weather sa Singapore? Hoping to go there by this year. \\
        & \textbf{DialoGPT:} It's been raining like crazy for the past few days. I was there last week and it was raining nonstop for the whole day. We were lucky enough to be in a place where it didn't rain that much. Singapore is one of the cleanest cities in the world when it comes to pollution. Don't worry too much about the pollution as it won't make that much of a big deal. \\
        & \textbf{User:} Ah ganun ba. Hindi na lang ako pupunta if that is the case. \\
        & \textbf{DialoGPT:} If you want to enjoy the cleanliness of the city then by all means go there. But if you just want to chill and gorge yourself, then go elsewhere. \\ 
        \hline
        \multirow{4}{\linewidth}{20\%} 
        & \textbf{User:} Kamusta yung weather sa Singapore? Hoping to go there by this year. \\
        & \textbf{DialoGPT:} It's been raining like crazy for the past few days. I was there last week and it was raining non stop for the whole day. We were lucky enough to have just enough time to get out of the car and onto the sidewalk. \\
        & \textbf{User:} Ah ganun ba, thanks for the info! Hindi nalang ako pupunta. \\
        & \textbf{DialoGPT:} You're welcome. Enjoy your trip. \\ 
        \hline
        \multirow{4}{\linewidth}{25\%} 
        & \textbf{User:} Kamusta yung weather sa Singapore? Hoping to go there by this year. \\
        & \textbf{DialoGPT:} Medyo malamig na ngayon dito sa singapore. Medyo mainit pero nakakapagod. \\
        & \textbf{User:} Ah ganun ba. Hindi na lang ako pupunta if that is the case. \\
        & \textbf{DialoGPT:} Yup, mainit talaga. \\ 
        \hline
        \multirow{4}{\linewidth}{30\%} 
        & \textbf{User:} Kamusta yung weather sa Singapore? Hoping to go there by this year. \\
        & \textbf{DialoGPT:}  It's been raining like crazy for the past few days. I was there last week and it was raining nonstop the whole time i was there. \\
        & \textbf{User:} Ah ganun ba. Hindi na lang ako pupunta if that is the case. \\
        & \textbf{DialoGPT:} You can try going there on a sunday. The weather is better during sundays. \\ 
        \hline
    \end{tabularx}
    \caption{\label{fig:iter1stylefashion} Travel \& Leisure Examples}
\end{figure*}




==> tables/table5-4.tex <==
\begin{figure}[!h]
\noindent\fbox{%
    \parbox{0.45\textwidth}{%
        \textbf{Domain:} Travel and Leisure  
        \newline
        \textbf{User}: What is the best way to commute in Germany?
        \newline
        \textbf{DialoGPT}: By bus.
        \newline        
        \textbf{User}: Bakit bus? Pangit ba yung train station nila?
        \newline
        \textbf{DialoGPT}: Medyo mahal nga.
        \newline
        \newline
        \textbf{Domain:} Visas and Immigration
        \newline
        \textbf{User}: Kailangan ba ng visa sa australia?
        \newline
        \textbf{DialoGPT}: Yes, kailangan ng visa.
        \newline
        \textbf{User}: Anong documents need?
        \newline
        \textbf{DialoGPT}: Passport, plane ticket, hotel booking.
        \newline
        \newline
        \textbf{Domain:} Body and Fitness
        \newline
        \textbf{User}: Ano yung workout routine mo?
        \newline
        \textbf{DialoGPT}: 5x5, squat, deadlift, bench press, military press
        \newline
        \textbf{User}: Araw-araw mo ba yan ginagawa?
        \newline
        \textbf{DialoGPT}: Hindi po araw araw
        \newline
        \newline
        \textbf{Domain:} Style and Fashion
        \newline
        \textbf{User}: Ano yung favorite product niyo sa uniqlo?
        \newline
        \textbf{DialoGPT}: Haven't tried any of their line. Their shirts are ok. nothing special. Their jeans are nice though.
        \newline
        \textbf{User}: Are there any brands you prefer besides unqilo?
        \newline
        \textbf{DialoGPT}: Uniqlo's jeans are ok, but i don't think you'd like them if you're a skinny person.
    }
}
\caption{Examples of conversations within the domain of the corpus.}
\label{fig:RelevantResponses}
\end{figure}

==> tables/table5-5.tex <==
\begin{figure}[!h]
\noindent\fbox{%
    \parbox{0.45\textwidth}{%
        \textbf{Example 1:}
        \newline
        \textbf{User}: Ano yung paboritong mong pelikula?
        \newline
        \textbf{DialoGPT}: Hindi ko alam kung ano itsura nung mga bulaklak na yan.
        \newline
        \textbf{User}: Paboritong bulaklak ko ay Sampaguita.
        \newline
        \textbf{DialoGPT}: Saan banda yan?
        \newline
        \newline
        \textbf{Example 2:}
        \newline
        \textbf{User}: Nakapagrehistro ka na bang bumoto?
        \newline
        \textbf{DialoGPT}: Hindi ko pa nakikita kung bakit nagkakamali ako.
        \newline
        \textbf{User}: Saan ka ba nagkakamali?
        \newline
        \textbf{DialoGPT}: Sa bahay.
        \newline
        \newline
        \textbf{Example 3:}
        \newline
        \textbf{User}: Mahilig ka ba magonline shopping?
        \newline
        \textbf{DialoGPT}: Hindi ko pa nakikita yung mga stores na nagbebenta ng toys from japan like lilo \& stitch, pooh, mickey \& others.
        \newline
        \textbf{User}: Ah mahilig ka pala sa mga toys.
        \newline
        \textbf{DialoGPT}: Yup. Mahilig ako sa toys ng japan.
    }%
}
\caption{Examples of conversations outside the domain of corpus.}
\label{fig:IrrelevantResponses}
\end{figure}
